Internal structure of incipient soot from acetylene pyrolysis obtained via molecular dynamics simulations

A series of reactive molecular dynamics simulations is used to study the internal structure of incipient soot particles obtained from acetylene pyrolysis. The simulations were performed using ReaxFF potential at four different temperatures. The resulting soot particles are cataloged and analyzed to obtain statistics of their mass, volume, density, C/H ratio, number of cyclic structures, and other features. A total of 3324 incipient soot particles were analyzed in this study. Based on their structural characteristics, the incipient soot particles are classified into two classes, referred to as type 1 and type 2 incipient soot particles in this work. The radial distribution of density, cyclic (5-, 6-, or 7-member rings) structures and C/H ratio inside the particles revealed a clear difference in the internal structure between type 1 and type 2 particles. These classes were further found to be well represented by the size of the particles with smaller particles in type 1 and larger particles in type 2. The radial distributions of ring structures, density, and C/H ratio indicated the presence of a dense core region in type 2 particles, whereas no clear evidence of the presence of a core was found in type 1 particles. In type 2 incipient soot particles, the boundary between the core and shell was found to be around 50%-60% of the particle radius of gyration.

==> preamble.tex <==
%\usepackage{epstopdf}% To incorporate .eps illustrations using PDFLaTeX, etc.
%\usepackage[caption=false]{subfig}% Support for small, `sub' figures and tables
%\usepackage[nolists,tablesfirst]{endfloat}% To `separate' figures and tables from text if required

%\usepackage[doublespacing]{setspace}% To produce a `double spaced' document if required
%\setlength\parindent{24pt}% To increase paragraph indentation when line spacing is doubled
%\setlength\bibindent{2em}% To increase hanging indent in bibliography when line spacing is doubled

%%%%%%%%%%%%%%%%%%%% Bibtex set up %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage[numbers,sort&compress]{natbib}% Citation support using natbib.sty
%\bibpunct[, ]{[}{]}{,}{n}{,}{,}% Citation support using natbib.sty
%\renewcommand\bibfont{\fontsize{10}{12}\selectfont}% Bibliography support using natbib.sty

%%%%%%%%%%%%%%%%%% Theore and Lemma etc. %%%%%%%%%%%%%%%%%%%%%
%\theoremstyle{plain}% Theorem-like structures provided by amsthm.sty
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}

%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{example}[theorem]{Example}

%\theoremstyle{remark}
%\newtheorem{remark}{Remark}
%\newtheorem{notation}{Notation}

%% This list environment is used for the references in the
%% Program Summary
%%
\newcounter{bla}
\newenvironment{refnummer}{%
   \list{[\arabic{bla}]}%
   {\usecounter{bla}%
      \setlength{\itemindent}{0pt}%
      \setlength{\topsep}{0pt}%
      \setlength{\itemsep}{0pt}%
      \setlength{\labelsep}{2pt}%
      \setlength{\listparindent}{0pt}%
      \settowidth{\labelwidth}{[9]}%
      \setlength{\leftmargin}{\labelwidth}%
      \addtolength{\leftmargin}{\labelsep}%
      \setlength{\rightmargin}{0pt}}}
{\endlist}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Others %%%%%%%%%%%%%%%%%%%%
%my own adjustments
\usepackage{lineno}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage[table,xcdraw]{xcolor}
%\usepackage{graphics}
%\usepackage{xkeyval}
% \usepackage{subfigure}
% \usepackage{subcaption}
\usepackage{subfig}
%\usepackage[graphicx]{realboxes}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{layout}
%\usepackage{multirow}
\usepackage{gensymb}
\usepackage{listings}

\lstset{
   breaklines=true,
   basicstyle=\ttfamily}

\usepackage{comment}
\usepackage{verbatim}
%\usepackage{verbatimbox}
%\usepackage{caption}
% \usepackage{subcaption}
%\captionsetup{compatibility=false}

%\usepackage{float}
%\usepackage{titlesec}
%\usepackage{pdflscape}
%\usepackage{adjustbox}
%\usepackage{rotating}
\usepackage{hyperref}
%\usepackage[figuresleft]{rotating}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
%\usepackage{textcomp}
%\usepackage{gensymb}

%\usepackage[tablesfirst,nomarkers,nolists]{endfloat}
%\DeclareDelayedFloatFlavor{sidewaystable}{table}
%\DeclareDelayedFloatFlavor{sidewaysfigure}{figure}
\usepackage{fancyvrb}
\usepackage[normalem]{ulem} %for strikethrough
\usepackage{enumitem}
% \renewcommand{\labelitemi}{$\circ$}
\renewcommand{\labelitemii}{$\circ$}
\renewcommand{\labelitemiii}{\tiny$\blacksquare$}
\renewcommand{\labelitemiv}{\tiny$\square$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Figure Location %%%%%%%%%%%%%%%%%

% \usepackage{multirow}
% \usepackage{graphicx}
% \graphicspath{{figures/}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Line Numbers %%%%%%%%%%%%%%%%%%

%\usepackage[modulo]{lineno}
%\linenumbers

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Random Text %%%%%%%%%%%%%%%%%%
%\usepackage{blindtext}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Version Control %%%%%%%%%%%%%%%%
\usepackage[table,xcdraw]{xcolor}
